Venereau-type polynomials as potential counterexamples

We study some properties of the Venereau polynomials b_m=y+x^m(xz+y(yu+z^2)), a sequence of proposed counterexamples to the Abhyankar-Sathaye embedding conjecture and the Dolgachev-Weisfeiler conjecture. It is well known that these are hyperplanes and residual coordinates, and for m at least 3, they are C[x]-coordinates. For m=1,2, it is only known that they are 1-stable C[x]-coordinates. We show that b_2 is in fact a C[x]-coordinate. We introduce the notion of Venereau-type polynomials, and show that these are all hyperplanes, and residual coordinates. We show that some of these Venereau-type polynomials are in fact C[x]-coordinates; the rest remain potential counterexamples to the embedding and other conjectures. For those that we show to be coordinates, we also show that any automorphism with one of them as a component is stably tame. The remainder are stably tame, 1-stable C[x]-coordinates.

==> PaxHeader/abstract2.tex <==
18 gid=1967921456
18 uid=1800138874
20 ctime=1347284563
20 atime=1348583934
24 SCHILY.dev=234881026
22 SCHILY.ino=1605222
18 SCHILY.nlink=1


==> PaxHeader/definitions.tex <==
18 gid=1967921456
18 uid=1800138874
20 ctime=1347284925
20 atime=1348583957
24 SCHILY.dev=234881026
22 SCHILY.ino=1605666
18 SCHILY.nlink=1


==> PaxHeader/introduction2.tex <==
18 gid=1967921456
18 uid=1800138874
20 ctime=1345209382
20 atime=1348583945
24 SCHILY.dev=234881026
22 SCHILY.ino=1510231
18 SCHILY.nlink=1


==> PaxHeader/venereaupoly2.tex <==
18 gid=1967921456
18 uid=1800138874
20 ctime=1347285076
20 atime=1348583964
24 SCHILY.dev=234881026
22 SCHILY.ino=1605733
18 SCHILY.nlink=1


==> PaxHeader/vtype2.tex <==
18 gid=1967921456
18 uid=1800138874
20 ctime=1347285926
20 atime=1348583973
24 SCHILY.dev=234881026
22 SCHILY.ino=1605930
18 SCHILY.nlink=1

